ODDR: Outlier Detection & Dimension Reduction Based Defense Against Adversarial Patches

Adversarial attacks present a significant challenge to the dependable deployment of machine learning models, with patch-based attacks being particularly potent. These attacks introduce adversarial perturbations in localized regions of an image, deceiving even well-trained models. In this paper, we propose Outlier Detection and Dimension Reduction (ODDR), a comprehensive defense strategy engineered to counteract patch-based adversarial attacks through advanced statistical methodologies. Our approach is based on the observation that input features corresponding to adversarial patches-whether naturalistic or synthetic-deviate from the intrinsic distribution of the remaining image data and can thus be identified as outliers. ODDR operates through a robust three-stage pipeline: Fragmentation, Segregation, and Neutralization. This model-agnostic framework is versatile, offering protection across various tasks, including image classification, object detection, and depth estimation, and is proved effective in both CNN-based and Transformer-based architectures. In the Fragmentation stage, image samples are divided into smaller segments, preparing them for the Segregation stage, where advanced outlier detection techniques isolate anomalous features linked to adversarial perturbations. The Neutralization stage then applies dimension reduction techniques to these outliers, effectively neutralizing the adversarial impact while preserving critical information for the machine learning task. Extensive evaluation on benchmark datasets against state-of-the-art adversarial patches underscores the efficacy of ODDR. Our method enhances model accuracy from 39.26% to 79.1% under the GoogleAp attack, outperforming leading defenses such as LGS (53.86%), Jujutsu (60%), and Jedi (64.34%).

==> sec/re_attack.tex <==
\section{Adaptive Attack}
\label{attack}

\subsection{Adversary access}

\subsection{Constrained Attack}

==> sec/related_works.tex <==
\section{Related Works}
\label{related}

There are two approaches to defense against such attacks: empirical defenses and certified defenses.

\textit{Empirical defenses:} \textbf{Localized Gradient Smoothing (LGS)} \cite{naseer2019local} first normalizes gradient values and then uses a moving window to identify high-density regions based on certain thresholds.
%Naseer et al. \cite{naseer2019local} propose local gradient smoothing (LGS) to neutralize the effect of adversarial patch pixels. They first perform normalization over the gradient values, and then use a moving window to identify high-density regions (based on certain thresholds), which will be smoothed out to suppress the influence of the adversarial pixels. \\
\textbf{Jujutsu} \cite{Jujutsu} focuses on localizing adversarial patches and distinguishing them from benign samples, and uses generative adversarial networks to reconstruct the “clean” examples from adversarial examples. 
\textbf{Jedi} \cite{jedi} is based on an input entropy analysis and recovering the image using inpaint.
%Chen et al. \cite{Jujutsu} propose Jujutsu to localize adversarial patch and distinguish it from benign samples, and uses generative adversarial networks to reconstruct the “clean” examples from adversarial examples. 
These defenses, while valuable, do come with certain limitations such as high false positive rates, 
poor detection rates, 

%: Some of these defense mechanisms struggle with reliably locating and identifying the exact position of the adversarial patch within an image. This limitation can hinder their effectiveness in precisely countering the attack.
%and/or low mitigation rate. 

%: Another challenge is the ability to mitigate the adversarial impact effectively while still allowing deep neural networks (DNNs) to make correct inferences on the adversarial examples. In some cases, these defenses might remove or alter important features, causing the model's performance to degrade even on benign samples.
%Limitations:
%High false positive rates: unable to correctly distinguish adversarial examples from clean samples.
%Poor detection rates: unable to reliably locate the patch.
%Low mitigation rate (robust accuracy):  unable to allow the DNNs to make correct inference on the adversarial examples as many important features are corrupted

\textit{Certified defenses:} \textbf{De-randomized smoothing (DS)} \cite{levine2020randomized} introduces a certified defense technique by building a smoothed classifier by ensembling local predictions made on pixel patches. \textbf{PatchGuard (PG)}\cite{xiang2021patchguard} uses enforcing a small receptive field within deep neural networks (DNNs) and secure feature aggregation.
%Levine et al. \cite{levine2020randomized} introduce de-randomized smoothing (DS) to build a smoothed classifier whose prediction is based on the ensemble of local prediction on pixel patches.\\
%Xiang et al. \cite{xiang2021patchguard} propose PatchGuard, a certified defense technique against patch attacks. The main idea is to enforce small receptive field in the DNNs, and secure feature aggregation by masking out the regions with the highest sum of class evidence (as these regions are more likely to be manipulated by adversarial patch to dominate the prediction).






==> sec/theory.tex <==
\section{Theoretical Background}
\label{theory}
%We discuss the basic theoretical fundamentals that form building blocks of the proposed ODDR scheme here. Firstly, we clearly define the threat model and the access that the attacker has to implement the attack. And then, we describe the two components of the defense mechanism, corresponding to identifying the patch and neutralizing it. 
In this section, we delve into the foundational theoretical principles that constitute the building blocks of the proposed ODDR scheme. We expound upon the dual components of the defense mechanism. %delineating the distinct stages involved in both identifying the adversarial patch and executing its subsequent neutralization. 
%---------------------------------------
\subsection{Segregating Input Features}
%---------------------------------------
%\textcolor{red}{TODO: Missing citations}

%Isolation Forest is used for outlier/anomaly detection
%Isolation Forest is an Unsupervised Learning technique (does not need label)
%Uses Binary Decision Trees bagging (resembles Random Forest, in supervised learning)
We use the Isolation Forest algorithm as a robust tool for detecting outliers and anomalies within datasets. Operating under the paradigm of Unsupervised Learning, this technique excels in scenarios where labeled data is unavailable, making it particularly versatile in diverse applications. Noteworthy is the algorithm's deployment of Binary Decision Trees through a bagging approach, drawing parallels to the well-known Random Forest technique employed in supervised learning. The core hypothesis guiding Isolation Forest is predicated on the assumption that anomalies represent a minority within the dataset, comprising fewer instances than their normal counterparts. Additionally, these anomalies are posited to possess attribute-values that diverge from those associated with normal instances. In simpler terms, anomalies are characterized as being both fewer in number and different from the rest of the samples \cite{IF}. This particularly makes it a good fit for detecting adversarial patches from input features of the test samples.
Leveraging these assumptions, Isolation Forest excels in isolating anomalies by constructing an ensemble of Binary Trees for a given dataset. Anomalies, given their distinctive nature, tend to exhibit shorter paths within these trees compared to normal instances \cite{IFextended}. 
%This inherent characteristic facilitates the effective isolation of anomalies, as their expedited descent toward the root of the tree distinguishes them from the majority of normal instances. In essence, Isolation Forest exploits the unique characteristics of anomalies to discern and segregate them from the broader dataset, making it a powerful tool in outlier detection and anomaly isolation \cite{IFextended}.
%Hypothesis:
%This method isolates anomalies from normal instances, for doing this the following assumptions for anomalies are made: They are a minority consisting of fewer instances, They have attribute-values that are different from normal instances. In other words, anomalies are “few and different.” 
%Because of these first two assumptions, anomalies are susceptible to be isolated and this makes them fall closer to the root of the tree. Isolation Forest builds an ensemble of Binary Trees for a given dataset. Anomalies, due to their nature, they have the shortest path in the trees than normal instances.
%Isolation Forest converges quickly with a very small number of trees and subsampling enables us to achieve good results while being computationally efficient. Isolation Forest recursively generates partitions on the dataset by randomly selecting a feature and then randomly selecting a split value for the feature. Presumably the anomalies need fewer random partitions to be isolated compared to "normal" points in the dataset, so the anomalies will be the points which have a smaller path length in the tree, path length being the number of edges traversed from the root node.

\subsection{Outlier Detection}

Let's formally define the mechanism of constructing an isolation tree for the purpose of detecting outliers. Consider a dataset $X = \{ x_1, \ldots, x_n \}$, comprising $n$ vectors representing instances from a multivariate distribution of dimension $d$.  %in order to construct the isolation tree, the dataset $X$ is recursively divided by randomly selected attribute $q$ and a threshold for the value to split $p$, up until one of the following three conditions appear:
To build the isolation tree, the dataset $X$ undergoes a recursive division process based on the random selection of an attribute $q$ and a corresponding threshold value $p$. This process continues until one of the following three conditions is met:

\begin{itemize}
    \item the isolation tree attains maximum permissible height
    \item $|X| = 1$
    \item the data in the dataset $X$ has equal values
\end{itemize}

%The objective of anomaly or outlier detection can be achieved if one can deduce a way to rank the samples reflecting degree of anomaly. This can be done by running a sorting algorithm on the path lengths or anomaly scores. This naturally necessitates the definition of the anomaly scores. 
The attainment of the objective in anomaly or outlier detection hinges on the ability to rank samples, reflecting their degree of anomaly. This ranking can be accomplished by applying a sorting algorithm to the path lengths or anomaly scores associated with each sample. Consequently, the definition of anomaly scores becomes imperative in this context. %Anomaly scores serve as a quantifiable measure, enabling the identification and prioritization of samples based on their deviation from the norm. This ranking mechanism is pivotal for effectively distinguishing anomalies and facilitating further analysis or action based on their level of abnormality.

%Path length $h(x)$ of a sample point $x$ may be defined as the measurement of the number of nodes that is needed by $x$ to traverse in the isolation tree from the root node, till the termination of the traversal at an external node. Utilizing the similarities in the structure of the isolation trees and the Binary Search Tree, it can be deduced that estimated average path length is same as that of an unsuccessful search in the Binary Search Tree. Now it is well known that for a dataset of $n$ samples, the average path length of an unsuccessful search is:

The path length $h(x)$ for a sample point $x$ is defined as the count of nodes that $x$ traverses in the isolation tree from the root node to the conclusion of the traversal at an external node. Drawing on the structural similarities between isolation trees and Binary Search Trees, it can be inferred that the estimated average path length aligns with that of an unsuccessful search in a Binary Search Tree. Well-established in the literature, it is known that for a dataset comprising $n$ samples, the average path length of an unsuccessful search is:
\begin{equation}
\label{path}
    c(n) = 2H(n-1)-(2(n-1)/n), 
\end{equation}
with $H(i)$ denoting the Harmonic number, estimated as $ln(i) + 0.57721567$ [Euler's constant]. Additionally, $c(n)$ represents the mean of $h(x)$ over $n$. Consequently, the anomaly score $s$ can be defined as:

\begin{equation}
\label{score}
    Score(x) = s(x,n) = 2^{-\frac{E(h(x))}{c(n)}}
\end{equation}

where $E(h(x))$ represents the mean of $h(x)$ derived from the isolation forest, which is constructed from multiple isolation trees. It follows that when $E(h(x)) \to c(n)$, $s \to 0.5$; when $E(h(x)) \to 0$, $s \to 1$; and when $E(h(x)) \to n-1$, $s \to 0$. 
%The interpretation of the anomaly score $s$ is that if the samples have an associated anomaly score near unity, then they are highly likely to be outliers, the ones with the score much smaller than $0.5$ are likely to belong to the distribution and if most of the samples return a score around the $0.5$ mark, then it is highly likely that there are not many outliers in the dataset. 
The interpretation of the anomaly score $s$ is as follows:
\begin{itemize}
    \item If the samples possess an anomaly score close to unity, they are highly likely to be outliers.
    \item Those with a score much smaller than $0.5$ are likely to belong to the distribution.
    \item If a significant portion of samples returns a score around the $0.5$ mark, it is highly probable that there are not many outliers in the dataset.
\end{itemize}



Isolation Forest exhibits swift convergence even with a minimal number of trees, and the incorporation of subsampling enhances its ability to yield favorable results while maintaining computational efficiency. The algorithm operates through a recursive process of generating partitions on the dataset, achieved by randomly selecting features and subsequently assigning random split values for these features. 
%An intriguing facet arises from the hypothesis that anomalies necessitate fewer random partitions for isolation compared to their "normal" counterparts in the dataset. Consequently, 
Anomalies are identified by their shorter path lengths within the tree structure, with path length denoting the number of edges traversed from the root node. 
%This characteristic enables Isolation Forest to efficiently and effectively discern anomalies, solidifying its position as a powerful tool for anomaly detection, particularly in datasets with high dimensionality.



\subsection{Dimension Reduction}
Dimension Reduction has been successfully used as a method of mitigating adversarial attacks \cite{cod_1, cod_2}. This technique maps the input into a lower dimensional space, preserving a chosen amount of variability, thereby getting rid of significant proportion of the adversarial noise. This is a standard technique that is used in linear algebra for decomposing a matrix, like the portions of images in our use-case, into components which are able to express the informational variability of the original matrix in useful forms \cite{freedman}. Intuitively, this projects the matrix on to an orthonormal basis and the variability within it is expressed as a linear combination of the components. 
At first, if we consider that an image (a coloured image has three channels and therefore three such matrices) is a $m$x$n$-matrix $M$, then one can use Singular Value Decomposition to factorize the same into $M = U \Sigma V^{T}$, where $U$ and $V$ are orthogonal matrices and $\Sigma = diag(\sigma_{1}, \ldots, \sigma_{r})$, where $r=min(m,n)$ such that $\sigma_{1} \geq \ldots \geq \sigma_{r} \geq 0$. In this case, the singular values are the $\sigma_{i}$s, and thereby we have the top $r$ columns of $V$ and $U$ being the right and left singular vectors respectively. This formulation is necessary for dimensionality reduction using Truncated Singular Value Decomposition as explained hereafter. 
For the matrix $M$ with a rank $r$, one can represent $M = U_{r} \Sigma_{r} V_{r}^{T}$ where $U_{r}$ and $V_{r}$ comprises of the left and right singular vectors. For any $k$, such that $(k <r)$, one can therefore obtain $M_{k}$, where $M_{k} = U_{k} \Sigma_{k} V^{T}_{k}$, which is lower rank approximation of the matrix. This is used in dimensionality reduction, facilitated by the fact that the singular values are so arranged such that they provide the ordering of the information contained in such truncated approximations.  
Specifically, in our implementation, we have used the proportion of the singular values as a surrogate to estimate the amount of information preserved upon the image mask $M$ being projected to a lower dimension. We have denoted this information preservation parameter as $inf$ and used it as a tuning parameter for our defense mechanism.
